Search for a critical point of strongly-interacting matter in central $^{40}$Ar +$^{45}$Sc collisions at 13$A$-75$A$ GeV/$c$ beam momentum

The critical point of strongly interacting matter is searched for at the CERN SPS by the NA61/SHINE experiment in central $^{40}$Ar +$^{45}$Sc collisions at 13$A$, 19$A$, 30$A$, 40$A$, and 75$A$ GeV/$c$. The dependence of the second-order scaled factorial moments of proton multiplicity distributions on the number of subdivisions in transverse momentum space is measured. The intermittency analysis uses statistically independent data sets for every subdivision in transverse and cumulative-transverse momentum variables. The results obtained do not indicate the searched intermittent pattern. An upper limit on the fraction of correlated protons and the intermittency index is obtained based on a comparison with the Power-law Model.

==> include/na61Authors.tex <==
% based on XML DB with time Thu Jan 19 15:27:22 2023
% Authors in alphabetical order.

\noindent
H.~Adhikary$^{\,13}$,
P.~Adrich$^{\,15}$,
K.K.~Allison$^{\,29}$,
N.~Amin$^{\,5}$,
E.V.~Andronov$^{\,25}$,
T.~Anti\'ci\'c$^{\,3}$,
I.-C.~Arsene$^{\,12}$,
M.~Bajda$^{\,16}$,
Y.~Balkova$^{\,18}$,
M.~Baszczyk$^{\,17}$,
D.~Battaglia$^{\,28}$,
A.~Bazgir$^{\,13}$,
S.~Bhosale$^{\,14}$,
M.~Bielewicz$^{\,15}$,
A.~Blondel$^{\,4}$,
M.~Bogomilov$^{\,2}$,
Y.~Bondar$^{\,13}$,
N.~Bostan$^{\,28}$,
A.~Brandin$^{\,24}$,
W.~Bryli\'nski$^{\,21}$,
J.~Brzychczyk$^{\,16}$,
M.~Buryakov$^{\,23}$,
A.F.~Camino$^{\,31}$,
M.~\'Cirkovi\'c$^{\,26}$,
~M.~Csanad~$^{\,7,8}$,
J.~Cybowska$^{\,21}$,
T.~Czopowicz$^{\,13,21}$,
C.~Dalmazzone$^{\,4}$,
N.~Davis$^{\,14}$,
A.~Dmitriev~$^{\,23}$,
P.~von~Doetinchem$^{\,30}$,
W.~Dominik$^{\,19}$,
P.~Dorosz$^{\,17}$,
J.~Dumarchez$^{\,4}$,
R.~Engel$^{\,5}$,
G.A.~Feofilov$^{\,25}$,
L.~Fields$^{\,28}$,
Z.~Fodor$^{\,7,20}$,
M.~Friend$^{\,9}$,
A.~Garibov$^{\,1}$,
M.~Ga\'zdzicki$^{\,13,6}$,
O.~Golosov$^{\,24}$,
V.~Golovatyuk~$^{\,23}$,
M.~Golubeva$^{\,22}$,
K.~Grebieszkow$^{\,21}$,
F.~Guber$^{\,22}$,
S.N.~Igolkin$^{\,25}$,
S.~Ilieva$^{\,2}$,
A.~Ivashkin$^{\,22}$,
A.~Izvestnyy$^{\,22}$,
K.~Kadija$^{\,3}$,
N.~Kargin$^{\,24}$,
N.~Karpushkin$^{\,22}$,
E.~Kashirin$^{\,24}$,
M.~Kie{\l}bowicz$^{\,14}$,
V.A.~Kireyeu$^{\,23}$,
H.~Kitagawa$^{\,10}$,
R.~Kolesnikov$^{\,23}$,
D.~Kolev$^{\,2}$,
Y.~Koshio$^{\,10}$,
V.N.~Kovalenko$^{\,25}$,
S.~Kowalski$^{\,18}$,
B.~Koz{\l}owski$^{\,21}$,
A.~Krasnoperov$^{\,23}$,
W.~Kucewicz$^{\,17}$,
M.~Kuchowicz$^{\,20}$,
M.~Kuich$^{\,19}$,
A.~Kurepin$^{\,22}$,
A.~L\'aszl\'o$^{\,7}$,
M.~Lewicki$^{\,20}$,
G.~Lykasov$^{\,23}$,
V.V.~Lyubushkin$^{\,23}$,
M.~Ma\'ckowiak-Paw{\l}owska$^{\,21}$,
Z.~Majka$^{\,16}$,
A.~Makhnev$^{\,22}$,
B.~Maksiak$^{\,15}$,
A.I.~Malakhov$^{\,23}$,
A.~Marcinek$^{\,14}$,
A.D.~Marino$^{\,29}$,
K.~Marton$^{\,7}$,
H.-J.~Mathes$^{\,5}$,
T.~Matulewicz$^{\,19}$,
V.~Matveev$^{\,23}$,
G.L.~Melkumov$^{\,23}$,
A.~Merzlaya$^{\,12}$,
{\L}.~Mik$^{\,17}$,
A.~Morawiec$^{\,16}$,
S.~Morozov$^{\,22}$,
Y.~Nagai~$^{\,8}$,
T.~Nakadaira$^{\,9}$,
M.~Naskr\k{e}t$^{\,20}$,
S.~Nishimori$^{\,9}$,
V.~Ozvenchuk$^{\,14}$,
O.~Panova$^{\,13}$,
V.~Paolone$^{\,31}$,
O.~Petukhov$^{\,22}$,
I.~Pidhurskyi$^{\,13,6}$,
R.~P{\l}aneta$^{\,16}$,
P.~Podlaski$^{\,19}$,
B.A.~Popov$^{\,23,4}$,
B.~Porfy$^{\,7,8}$,
M.~Posiada{\l}a-Zezula$^{\,19}$,
D.S.~Prokhorova$^{\,25}$,
D.~Pszczel$^{\,15}$,
S.~Pu{\l}awski$^{\,18}$,
J.~Puzovi\'c$^{\,26}$,
R.~Renfordt$^{\,18}$,
L.~Ren$^{\,29}$,
V.Z.~Reyna~Ortiz$^{\,13}$,
D.~R\"ohrich$^{\,11}$,
E.~Rondio$^{\,15}$,
M.~Roth$^{\,5}$,
{\L}.~Rozp{\l}ochowski$^{\,14}$,
B.T.~Rumberger$^{\,29}$,
M.~Rumyantsev$^{\,23}$,
A.~Rustamov$^{\,1,6}$,
M.~Rybczynski$^{\,13}$,
A.~Rybicki$^{\,14}$,
K.~Sakashita$^{\,9}$,
K.~Schmidt$^{\,18}$,
A.Yu.~Seryakov$^{\,25}$,
P.~Seyboth$^{\,13}$,
U.A.~Shah$^{\,13}$,
Y.~Shiraishi$^{\,10}$,
A.~Shukla$^{\,30}$,
M.~S{\l}odkowski$^{\,21}$,
P.~Staszel$^{\,16}$,
G.~Stefanek$^{\,13}$,
J.~Stepaniak$^{\,15}$,
M.~Strikhanov$^{\,24}$,
H.~Str\"obele$^{\,6}$,
T.~\v{S}u\v{s}a$^{\,3}$,
{\L}.~\'Swiderski$^{\,15}$,
J.~Szewi\'nski$^{\,15}$,
R.~Szukiewicz$^{\,20}$,
A.~Taranenko$^{\,24}$,
A.~Tefelska$^{\,21}$,
D.~Tefelski$^{\,21}$,
V.~Tereshchenko$^{\,23}$,
A.~Toia$^{\,6}$,
R.~Tsenov$^{\,2}$,
L.~Turko$^{\,20}$,
T.S.~Tveter$^{\,12}$,
M.~Unger$^{\,5}$,
M.~Urbaniak$^{\,18}$,
F.F.~Valiev$^{\,25}$,
D.~Veberi\v{c}$^{\,5}$,
V.V.~Vechernin$^{\,25}$,
V.~Volkov$^{\,22}$,
A.~Wickremasinghe$^{\,27}$,
K.~W\'ojcik$^{\,18}$,
O.~Wyszy\'nski$^{\,13}$,
A.~Zaitsev$^{\,23}$,
E.D.~Zimmerman$^{\,29}$,
A.~Zviagina$^{\,25}$, and
R.~Zwaska$^{\,27}$


==> include/na61Institutions.tex <==
% based on XML DB with time Thu Jan 19 15:27:22 2023
% Institutes in alphabetical order.

\noindent
$^{1}$~National Nuclear Research Center, Baku, Azerbaijan\\
$^{2}$~Faculty of Physics, University of Sofia, Sofia, Bulgaria\\
$^{3}$~Ru{\dj}er Bo\v{s}kovi\'c Institute, Zagreb, Croatia\\
$^{4}$~LPNHE, University of Paris VI and VII, Paris, France\\
$^{5}$~Karlsruhe Institute of Technology, Karlsruhe, Germany\\
$^{6}$~University of Frankfurt, Frankfurt, Germany\\
$^{7}$~Wigner Research Centre for Physics, Budapest, Hungary\\
$^{8}$~E\"otv\"os Lor\'and University, Budapest, Hungary\\
$^{9}$~Institute for Particle and Nuclear Studies, Tsukuba, Japan\\
$^{10}$~Okayama University, Japan\\
$^{11}$~University of Bergen, Bergen, Norway\\
$^{12}$~University of Oslo, Oslo, Norway\\
$^{13}$~Jan Kochanowski University, Poland\\
$^{14}$~Institute of Nuclear Physics, Polish Academy of Sciences, Cracow, Poland\\
$^{15}$~National Centre for Nuclear Research, Warsaw, Poland\\
$^{16}$~Jagiellonian University, Cracow, Poland\\
$^{17}$~AGH - University of Science and Technology, Cracow, Poland\\
$^{18}$~University of Silesia, Katowice, Poland\\
$^{19}$~University of Warsaw, Warsaw, Poland\\
$^{20}$~University of Wroc{\l}aw,  Wroc{\l}aw, Poland\\
$^{21}$~Warsaw University of Technology, Warsaw, Poland\\
$^{22}$~Institute for Nuclear Research, Moscow, Russia\\
$^{23}$~Joint Institute for Nuclear Research, Dubna, Russia\\
$^{24}$~National Research Nuclear University (Moscow Engineering Physics Institute), Moscow, Russia\\
$^{25}$~St. Petersburg State University, St. Petersburg, Russia\\
$^{26}$~University of Belgrade, Belgrade, Serbia\\
$^{27}$~Fermilab, Batavia, USA\\
$^{28}$~University of Notre Dame, Notre Dame , USA\\
$^{29}$~University of Colorado, Boulder, USA\\
$^{30}$~University of Hawaii at Manoa, USA\\
$^{31}$~University of Pittsburgh, Pittsburgh, USA\\

